Gradual Certified Programming in Coq

Expressive static typing disciplines are a powerful way to achieve high-quality software. However, the adoption cost of such techniques should not be under-estimated. Just like gradual typing allows for a smooth transition from dynamically-typed to statically-typed programs, it seems desirable to support a gradual path to certified programming. We explore gradual certified programming in Coq, providing the possibility to postpone the proofs of selected properties, and to check "at runtime" whether the properties actually hold. Casts can be integrated with the implicit coercion mechanism of Coq to support implicit cast insertion a la gradual typing. Additionally, when extracting Coq functions to mainstream languages, our encoding of casts supports lifting assumed properties into runtime checks. Much to our surprise, it is not necessary to extend Coq in any way to support gradual certified programming. A simple mix of type classes and axioms makes it possible to bring gradual certified programming to Coq in a straightforward manner.

==> DecidableExtns.tex <==
\coqlibrary{Casts.DecidableExtns}{Library }{Casts.DecidableExtns}

\begin{coqdoccode}
\coqdocemptyline
\coqdocemptyline
\end{coqdoccode}
The \coqref{Casts.DecidableExtns.Decidable}{\coqdocrecord{Decidable}} type class: \begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Class} \coqdef{Casts.DecidableExtns.Decidable}{Decidable}{\coqdocrecord{Decidable}} (\coqdocvar{A} : \coqdockw{Prop}) := \coqdef{Casts.DecidableExtns.dec}{dec}{\coqdocprojection{dec}} : \coqdocvariable{A} \coqexternalref{:type scope:x '+' x}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocnotation{+}} \coqexternalref{:type scope:x '+' x}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocnotation{(}}\coqexternalref{:type scope:'x7E' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{\ensuremath{\lnot}}} \coqdocvariable{A}\coqexternalref{:type scope:x '+' x}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocnotation{)}}.\coqdoceol
\coqdocemptyline
\coqdocemptyline
\end{coqdoccode}
\subsection{Basic boolean reflection}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable bool}{Decidable\_bool}{\coqdocinstance{Decidable\_bool}} (\coqdocvar{t} : \coqexternalref{bool}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{bool}}) : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{Is true}{http://coq.inria.fr/stdlib/Coq.Bool.Bool}{\coqdocdefinition{Is\_true}} \coqdocvariable{t}) :=\coqdoceol
\coqdocindent{1.00em}
\coqdockw{match} \coqdocvar{t} \coqdockw{with}\coqdoceol
\coqdocindent{2.00em}
\ensuremath{|} \coqexternalref{true}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{true}} \ensuremath{\Rightarrow} \coqexternalref{inl}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inl}} \coqexternalref{I}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocconstructor{I}}\coqdoceol
\coqdocindent{2.00em}
\ensuremath{|} \coqexternalref{false}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{false}} \ensuremath{\Rightarrow} \coqexternalref{inr}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inr}} \coqexternalref{id}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocdefinition{id}}\coqdoceol
\coqdocindent{1.00em}
\coqdockw{end}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsection{Boolean reflection with proven relation to a proposition}


 \label{app:bool_refl}
\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Class} \coqdef{Casts.DecidableExtns.Decidable relate}{Decidable\_relate}{\coqdocrecord{Decidable\_relate}} (\coqdocvar{P} : \coqdockw{Prop}) := \{\coqdoceol
\coqdocindent{1.00em}
\coqdef{Casts.DecidableExtns.Decidable witness}{Decidable\_witness}{\coqdocprojection{Decidable\_witness}} : \coqexternalref{bool}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{bool}};\coqdoceol
\coqdocindent{1.00em}
\coqdef{Casts.DecidableExtns.Decidable spec}{Decidable\_spec}{\coqdocprojection{Decidable\_spec}} : \coqref{Casts.DecidableExtns.Decidable witness}{\coqdocmethod{Decidable\_witness}} \coqexternalref{:type scope:x '=' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{=}} \coqexternalref{true}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{true}} \coqexternalref{:type scope:x '<->' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{\ensuremath{\leftrightarrow}}} \coqdocvariable{P}\coqdoceol
\coqdocnoindent
\}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Dec relate Decidable}{Dec\_relate\_Decidable}{\coqdocinstance{Dec\_relate\_Decidable}} \coqdocvar{P} (\coqdocvar{HP}: \coqref{Casts.DecidableExtns.Decidable relate}{\coqdocclass{Decidable\_relate}} \coqdocvariable{P}) : \coqdoceol
\coqdocindent{1.00em}
\coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P}.\coqdoceol
\coqdocnoindent
\coqdoctac{destruct} \coqdocvar{HP} \coqdockw{as} [\coqdocvar{witness} \coqdocvar{spec}]. \coqdoctac{destruct} \coqdocvar{witness}.\coqdoceol
\coqdocnoindent
- \coqdoctac{left}. \coqdoctac{exact} (\coqexternalref{proj1}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdoclemma{proj1}} \coqdocvar{spec} \coqexternalref{eq refl}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocconstructor{eq\_refl}}).\coqdoceol
\coqdocnoindent
- \coqdoctac{right}. \coqdoctac{intro} \coqdocvar{p}. \coqdoctac{pose} (\coqexternalref{proj2}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdoclemma{proj2}} \coqdocvar{spec} \coqdocvar{p}). \coqdoctac{inversion} \coqdocvar{e}.\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocemptyline
\coqdocemptyline
\end{coqdoccode}
\subsection{Decidable equality}



 A type class for types with decidable equality: \begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Class} \coqdef{Casts.DecidableExtns.EqDecidable}{EqDecidable}{\coqdocrecord{EqDecidable}} (\coqdocvar{A} : \coqdockw{Type}) := \{ \coqdoceol
\coqdocindent{1.00em}
\coqdef{Casts.DecidableExtns.eq dec}{eq\_dec}{\coqdocprojection{eq\_dec}} : \coqdockw{\ensuremath{\forall}} \coqdocvar{a} \coqdocvar{b} : \coqdocvariable{A}, \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqdocvariable{a} \coqexternalref{:type scope:x '=' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{=}} \coqdocvariable{b}) \coqdoceol
\coqdocnoindent
\}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsubsection{Instances for \texorpdfstring{\protect\coqexternalref{bool}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{bool}}}{bool}}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable eq bool}{Decidable\_eq\_bool}{\coqdocinstance{Decidable\_eq\_bool}} : \coqdockw{\ensuremath{\forall}} (\coqdocvar{x} \coqdocvar{y} : \coqexternalref{bool}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{bool}}), \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{eq}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{eq}} \coqdocvariable{x} \coqdocvariable{y}).\coqdoceol
\coqdocnoindent
\coqdoctac{intros}. \coqdoctac{destruct} \coqdocvar{x}, \coqdocvar{y}; \coqdoctac{try} (\coqdoctac{left} ;\coqdoctac{reflexivity}); \coqdoceol
\coqdocindent{4.00em}
\coqdoctac{try} (\coqdoctac{right}; \coqdoctac{intro} \coqdocvar{H}; \coqdoctac{inversion} \coqdocvar{H}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.EqDecidable bool}{EqDecidable\_bool}{\coqdocinstance{EqDecidable\_bool}} : \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqexternalref{bool}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{bool}} := \coqdoceol
\coqdocindent{1.00em}
\{ \coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} := \coqref{Casts.DecidableExtns.Decidable eq bool}{\coqdocinstance{Decidable\_eq\_bool}} \}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsubsection{Instances for \texorpdfstring{\protect\coqexternalref{nat}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{nat}}}{nat}}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable eq nat}{Decidable\_eq\_nat}{\coqdocinstance{Decidable\_eq\_nat}} : \coqdockw{\ensuremath{\forall}} (\coqdocvar{x} \coqdocvar{y} : \coqexternalref{nat}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{nat}}), \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{eq}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{eq}} \coqdocvariable{x} \coqdocvariable{y}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.EqDecidable nat}{EqDecidable\_nat}{\coqdocinstance{EqDecidable\_nat}} : \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqexternalref{nat}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{nat}} := \coqdoceol
\coqdocindent{1.00em}
\{ \coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} := \coqref{Casts.DecidableExtns.Decidable eq nat}{\coqdocinstance{Decidable\_eq\_nat}} \}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsubsection{Instances for \texorpdfstring{\protect\coqexternalref{list}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{list}}}{list}}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable eq list}{Decidable\_eq\_list}{\coqdocinstance{Decidable\_eq\_list}} : \coqdockw{\ensuremath{\forall}} \coqdocvar{A} (\coqdocvar{HA}: \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqdocvariable{A}) \coqdoceol
\coqdocindent{1.00em}
(\coqdocvar{x} \coqdocvar{y}: \coqexternalref{list}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{list}} \coqdocvariable{A}), \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{eq}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{eq}} \coqdocvariable{x} \coqdocvariable{y}).\coqdoceol
\coqdocnoindent
\coqdoctac{intros} \coqdocvar{A} \coqdocvar{HA}. \coqdoctac{induction} \coqdocvar{x}.\coqdoceol
\coqdocnoindent
- \coqdoctac{destruct} \coqdocvar{y}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{left}; \coqdoctac{reflexivity}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{right}; \coqdoctac{intro} \coqdocvar{H}; \coqdoctac{inversion} \coqdocvar{H}.\coqdoceol
\coqdocnoindent
- \coqdoctac{induction} \coqdocvar{y}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{right}; \coqdoctac{intro} \coqdocvar{H}; \coqdoctac{inversion} \coqdocvar{H}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{case} (\coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} \coqdocvar{a} \coqdocvar{a0}); \coqdoctac{intro} \coqdocvar{H}.\coqdoceol
\coqdocindent{2.00em}
\ensuremath{\times} \coqdoctac{case} (\coqdocvar{IHx} \coqdocvar{y}); \coqdoctac{intro} \coqdocvar{Hl}.\coqdoceol
\coqdocindent{3.00em}
\coqdoctac{left}. \coqdoctac{rewrite} \coqdocvar{H}. \coqdoctac{rewrite} \coqdocvar{Hl}. \coqdoctac{reflexivity}.\coqdoceol
\coqdocindent{3.00em}
\coqdoctac{right}. \coqdoctac{rewrite} \coqdocvar{H}. \coqdoctac{unfold} \coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}} \coqdoctac{in} *.\coqdoceol
\coqdocindent{3.00em}
\coqdoctac{intro} \coqdocvar{Hc}. \coqdoctac{inversion} \coqdocvar{Hc}. \coqdoctac{exact} (\coqdocvar{Hl} \coqdocvar{H1}).\coqdoceol
\coqdocindent{2.00em}
\ensuremath{\times} \coqdoctac{right}. \coqdoctac{unfold} \coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}} \coqdoctac{in} *.\coqdoceol
\coqdocindent{3.00em}
\coqdoctac{intro} \coqdocvar{Hc}. \coqdoctac{inversion} \coqdocvar{Hc}. \coqdoctac{exact} (\coqdocvar{H} \coqdocvar{H1}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.EqDecidable list}{EqDecidable\_list}{\coqdocinstance{EqDecidable\_list}} : \coqdoceol
\coqdocindent{1.00em}
\coqdockw{\ensuremath{\forall}} \coqdocvar{A} (\coqdocvar{HA}: \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqdocvariable{A}), \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} (\coqexternalref{list}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{list}} \coqdocvariable{A}) := \coqdoceol
\coqdocindent{2.00em}
\{ \coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} := \coqref{Casts.DecidableExtns.Decidable eq list}{\coqdocinstance{Decidable\_eq\_list}} \coqdocvar{HA} \}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsubsection{Instances for \texorpdfstring{\protect\coqexternalref{option}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{option}}}{option}}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable eq option}{Decidable\_eq\_option}{\coqdocinstance{Decidable\_eq\_option}} : \coqdockw{\ensuremath{\forall}} \coqdocvar{A} (\coqdocvar{HA}: \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqdocvariable{A}) \coqdoceol
\coqdocindent{1.00em}
(\coqdocvar{x} \coqdocvar{y}: \coqexternalref{option}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{option}} \coqdocvariable{A}), \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{eq}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{eq}} \coqdocvariable{x} \coqdocvariable{y}).\coqdoceol
\coqdocnoindent
\coqdoctac{intros}. \coqdoctac{destruct} \coqdocvar{x}; \coqdoctac{destruct} \coqdocvar{y}.\coqdoceol
\coqdocnoindent
- \coqdoctac{case} (\coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} \coqdocvar{a} \coqdocvar{a0}); \coqdoctac{intro} \coqdocvar{H}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{left}. \coqdoctac{rewrite} \coqdocvar{H}. \coqdoctac{reflexivity}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{right}. \coqdoctac{unfold} \coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}} \coqdoctac{in} *. \coqdoctac{intro} \coqdocvar{Hc}. \coqdoctac{inversion} \coqdocvar{Hc}.\coqdoceol
\coqdocindent{2.00em}
\coqdoctac{exact} (\coqdocvar{H} \coqdocvar{H1}).\coqdoceol
\coqdocnoindent
- \coqdoctac{right}. \coqdoctac{unfold} \coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}}. \coqdoctac{intro} \coqdocvar{Hc}. \coqdoctac{inversion} \coqdocvar{Hc}.\coqdoceol
\coqdocnoindent
- \coqdoctac{right}. \coqdoctac{unfold} \coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}}. \coqdoctac{intro} \coqdocvar{Hc}. \coqdoctac{inversion} \coqdocvar{Hc}.\coqdoceol
\coqdocnoindent
- \coqdoctac{left}. \coqdoctac{reflexivity}.\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.EqDecidable option}{EqDecidable\_option}{\coqdocinstance{EqDecidable\_option}} :\coqdoceol
\coqdocindent{1.00em}
\coqdockw{\ensuremath{\forall}} \coqdocvar{A} (\coqdocvar{HA}: \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} \coqdocvariable{A}), \coqref{Casts.DecidableExtns.EqDecidable}{\coqdocclass{EqDecidable}} (\coqexternalref{option}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{option}} \coqdocvariable{A}) := \coqdoceol
\coqdocindent{2.00em}
\{ \coqref{Casts.DecidableExtns.eq dec}{\coqdocmethod{eq\_dec}} := \coqref{Casts.DecidableExtns.Decidable eq option}{\coqdocinstance{Decidable\_eq\_option}} \coqdocvar{HA} \}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsection{Logical combination instances}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable and}{Decidable\_and}{\coqdocinstance{Decidable\_and}} \coqdocvar{P} \coqdocvar{Q} (\coqdocvar{HP} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P}) \coqdoceol
\coqdocindent{0.50em}
(\coqdocvar{HQ} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{Q}) : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqdocvariable{P} \coqexternalref{:type scope:x '/x5C' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{\ensuremath{\land}}} \coqdocvariable{Q}).\coqdoceol
\coqdocnoindent
\coqdoctac{destruct} \coqdocvar{HP}.\coqdoceol
\coqdocnoindent
- \coqdoctac{destruct} \coqdocvar{HQ}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{exact} (\coqexternalref{inl}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inl}} (\coqexternalref{conj}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocconstructor{conj}} \coqdocvar{p} \coqdocvar{q})).\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{apply} \coqexternalref{inr}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inr}}. \coqdoctac{intro} \coqdocvar{H}. \coqdoctac{exact} (\coqdocvar{n} (\coqexternalref{proj2}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdoclemma{proj2}} \coqdocvar{H})).\coqdoceol
\coqdocnoindent
- \coqdoctac{apply} \coqexternalref{inr}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inr}}. \coqdoctac{intro} \coqdocvar{H}. \coqdoctac{exact} (\coqdocvar{n} (\coqexternalref{proj1}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdoclemma{proj1}} \coqdocvar{H})).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable or}{Decidable\_or}{\coqdocinstance{Decidable\_or}} \coqdocvar{P} \coqdocvar{Q} (\coqdocvar{HP} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P})\coqdoceol
\coqdocindent{4.00em}
(\coqdocvar{HQ} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{Q}) : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqdocvariable{P} \coqexternalref{:type scope:x 'x5C/' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{\ensuremath{\lor}}} \coqdocvariable{Q}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable not}{Decidable\_not}{\coqdocinstance{Decidable\_not}} \coqdocvar{P} (\coqdocvar{HP} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P}) : \coqdoceol
\coqdocindent{1.00em}
\coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqexternalref{not}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocdefinition{not}} \coqdocvariable{P}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable implies}{Decidable\_implies}{\coqdocinstance{Decidable\_implies}} \coqdocvar{P} \coqdocvar{Q} (\coqdocvar{HP} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P}) \coqdoceol
\coqdocindent{1.00em}
(\coqdocvar{HQ} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{Q}) : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqdocvariable{P} \coqexternalref{:type scope:x '->' x}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocnotation{\ensuremath{\rightarrow}}} \coqdocvariable{Q}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable True}{Decidable\_True}{\coqdocinstance{Decidable\_True}} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqexternalref{True}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{True}} := \coqexternalref{inl}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inl}} \coqexternalref{I}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocconstructor{I}}.\coqdoceol
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable False}{Decidable\_False}{\coqdocinstance{Decidable\_False}} : \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqexternalref{False}{http://coq.inria.fr/stdlib/Coq.Init.Logic}{\coqdocinductive{False}} := \coqexternalref{inr}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inr}} \coqexternalref{id}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocdefinition{id}}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsection{Some arithmetic}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable le nat}{Decidable\_le\_nat}{\coqdocinstance{Decidable\_le\_nat}} : \coqdockw{\ensuremath{\forall}} (\coqdocvar{x} \coqdocvar{y} : \coqexternalref{nat}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocinductive{nat}}), \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} (\coqdocvariable{x} \coqexternalref{:nat scope:x '<=' x}{http://coq.inria.fr/stdlib/Coq.Init.Peano}{\coqdocnotation{\ensuremath{\le}}} \coqdocvariable{y}).\coqdoceol
\coqdocnoindent
\coqdoctac{induction} \coqdocvar{x}.\coqdoceol
\coqdocnoindent
- \coqdoctac{destruct} \coqdocvar{y}.\coqdoceol
\coqdocindent{0.50em}
+ \coqdoctac{left}. \coqdoctac{apply} \coqexternalref{le 0 n}{http://coq.inria.fr/stdlib/Coq.Arith.Le}{\coqdocabbreviation{le\_0\_n}}.\coqdoceol
\coqdocindent{0.50em}
+ \coqdoctac{left}. \coqdoctac{apply} \coqexternalref{le S}{http://coq.inria.fr/stdlib/Coq.Init.Peano}{\coqdocconstructor{le\_S}}, \coqexternalref{le 0 n}{http://coq.inria.fr/stdlib/Coq.Arith.Le}{\coqdocabbreviation{le\_0\_n}}.\coqdoceol
\coqdocnoindent
- \coqdoctac{induction} \coqdocvar{y}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{right}. \coqdoctac{apply} \coqexternalref{le Sn 0}{http://coq.inria.fr/stdlib/Coq.Arith.Le}{\coqdocabbreviation{le\_Sn\_0}}.\coqdoceol
\coqdocindent{1.00em}
+ \coqdoctac{case} (\coqdocvar{IHx} \coqdocvar{y}). \coqdoctac{intro} \coqdocvar{H}. \coqdoctac{left}. \coqdoctac{exact} (\coqexternalref{le n S}{http://coq.inria.fr/stdlib/Coq.Arith.Le}{\coqdoclemma{le\_n\_S}} \coqdocvar{\_} \coqdocvar{\_} \coqdocvar{H}).\coqdoceol
\coqdocindent{2.00em}
\coqdoctac{intro} \coqdocvar{H}; \coqdoctac{right}. \coqdoctac{intro}. \coqdoctac{apply} \coqdocvar{H}. \coqdoctac{exact} (\coqexternalref{le S n}{http://coq.inria.fr/stdlib/Coq.Arith.Le}{\coqdoclemma{le\_S\_n}} \coqdocvar{\_} \coqdocvar{\_} \coqdocvar{H0}).\coqdoceol
\coqdocnoindent
\coqdockw{Defined}.\coqdoceol
\coqdocemptyline
\end{coqdoccode}
\subsection{Decidability of proven properties}

\begin{coqdoccode}
\coqdocemptyline
\coqdocnoindent
\coqdockw{Instance} \coqdef{Casts.DecidableExtns.Decidable proven}{Decidable\_proven}{\coqdocinstance{Decidable\_proven}} (\coqdocvar{P} : \coqdockw{Prop}) (\coqdocvar{ev} :  \coqdocvariable{P}):  \coqref{Casts.DecidableExtns.Decidable}{\coqdocclass{Decidable}} \coqdocvariable{P} :=\coqdoceol
\coqdocindent{1.00em}
\coqexternalref{inl}{http://coq.inria.fr/stdlib/Coq.Init.Datatypes}{\coqdocconstructor{inl}} \coqdocvar{ev}.\coqdoceol
\coqdocemptyline
\coqdocemptyline
\end{coqdoccode}

